The Definition and Measurement of the Topological Entropy per Unit Volume in Parabolic PDE's

We define the topological entropy per unit volume in parabolic PDE's such as the complex Ginzburg-Landau equation, and show that it exists, and is bounded by the upper Hausdorff dimension times the maximal expansion rate. We then give a constructive implementation of a bound on the inertial range of such equations. Using this bound, we are able to propose a finite sampling algorithm which allows (in principle) to measure this entropy from experimental data.

==> fig.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point       -.31       8.20 {\clap{$t$}}
\point       7.55        .14 {\rlap{$x$}}
\point       3.12       8.16 {\clap{$L$}}
\point       3.12       -.64 {\clap{$L+\BX(E)/\epsilon$}}
\point       5.69       8.04 {\clap{$\delta_*$}}
\point       7.39       5.39 {\rlap{$\tau_*$}}
\point       6.99       3.79 {\rlap{$\tau_*\BX(GGG)\log(1/\epsilon)$}}
 }}

